Probabilistic Mobility Load Balancing for Multi-band 5G and Beyond Networks

The ever-increasing demand for data services and the proliferation of user equipment (UE) have resulted in a significant rise in the volume of mobile traffic. Moreover, in multi-band networks, non-uniform traffic distribution among different operational bands can lead to congestion, which can adversely impact the user's quality of experience. Load balancing is a critical aspect of network optimization, where it ensures that the traffic is evenly distributed among different bands, avoiding congestion and ensuring better user experience. Traditional load balancing approaches rely only on the band channel quality as a load indicator and to move UEs between bands, which disregards the UE's demands and the band resource, and hence, leading to a suboptimal balancing and utilization of resources. To address this challenge, we propose an event-based algorithm, in which we model the load balancing problem as a multi-objective stochastic optimization, and assign UEs to bands in a probabilistic manner. The goal is to evenly distribute traffic across available bands according to their resources, while maintaining minimal number of inter-frequency handovers to avoid the signaling overhead and the interruption time. Simulation results show that the proposed algorithm enhances the network's performance and outperforms traditional load balancing approaches in terms of throughput and interruption time.

==> data-analysis.tex <==
% \textcolor{gray}{Di: I feel we jumped into these details too quickly. Can we add one sentence to introduce the main focus of experiment part.} 
%This section presents the evaluation of our policy reuse framework. 
% In order to create various traffic scenarios, we collected a proprietary dataset of hourly communication traffic from an existing communication network over one week. In this dataset, there are 21 sectors and each sector has 4 cells with different frequencies and capacities. This dataset was used to tune a proprietary system-level network simulator so that it mimicks the real-world traffic conditions. 


We collected a proprietary dataset of hourly communication traffic from an existing communication network over one week. In this dataset, there are 21 sectors and each sector has 4 cells with different frequencies and capacities. This dataset was used to tune a proprietary system-level network simulator so that it mimics real-world traffic conditions. Details about the dataset and simulator are presented in Section~\ref{sec:traffic-analysis} and~\ref{sec:simulator}, respectively. Section~\ref{sec:baselines} lists the baselines that we use to compare our proposed method. Section~\ref{sec:policy-bank-analysis} constructs and analyses the policy bank that we obtained using simulated scenarios. Finally, Section~\ref{sec:policy-sector-training} and~\ref{sec:policy-sector-result} present our experiment with the policy selector and its performance evaluation.

%Our experiment studies load balancing on these traffic scenarios. Section~\ref{sec:traffic-analysis} presents these traffic scenarios and their clustering in detail. 
%
%To enable the RL algorithm to interact with a simulated environment, we recreate the real-world scenarios within a proprietary system-level network simulator by tuning the simulator's configurations so that it mimics real-world traffic conditions. 
%For each scenario, the configuration that results in a traffic condition matching the closest to the real-world data is kept. 
% More details about the simulator are presented in Section~\ref{sec:simulator}.

%Section~\ref{sec:baselines} presents the baseline methods we use to compare the effectiveness of our proposed framework. In Section~\ref{sec:policy-bank-analysis}, we investigate the performance of the policies in our policy bank on each traffic scenario. The high performance of policies on novel traffic scenarios similar to the traffic scenario seen during training further supports the need for a policy selector. Finally, we explain in detail our experiments using the policy selector in Section~\ref{sec:policy-sector-training} and present its results in Section~\ref{sec:policy-sector-result}.

\begin{figure}[t]
\centering
\begin{tabular}{c}
\includegraphics[width=0.7\columnwidth]{Figures/21sec-rl-analysis_train_group2.png} \\
(a) Average reward on the training scenarios \\
~\\
\includegraphics[width=0.7\columnwidth]{Figures/21sec-rl-analysis_test_group2.png} \\
(b)  Average reward on the testing scenarios \\
\end{tabular}
    \caption{Comparison of the average reward over one week between policies in the policy bank $\Pi$ (orange), the policy $\tilde{\pi}$ trained on all scenarios in $\mathcal{X}$ (blue), and BasicLB (green) across training and testing scenarios. For the policy bank evaluation (orange), we show the mean and indicate the minimum and maximum with error bars.}
    \label{fig:rl_policy_21_sec}
\end{figure}

\subsection{Traffic clustering and analysis}
\label{sec:traffic-analysis}
%\textcolor{gray}{Jimmy: I think we need to add 1 sentence here stating the overall purpose of this subsection. For example, something like "In this section we analyze the three predominant groups of network conditions...blah blah blah, by analyzing the distribution of traffic among various cells....". I think you can write something more accurate than me. } 
% Load balancing aims to move UEs from high traffic cells to low traffic cells to improve the overall efficiency of the network. %Various factors related to the environment, time and the system hardware can describe the traffic condition of a cell. 
%In this section, we conduct preparatory analysis to construct a diverse set of training scenarios with which we use to build our policy bank. 
To identify different types of traffic, we applied the K-Means clustering algorithm to the daily traffic condition described by three traffic-related factors: the number of active UEs, network throughput, and 
% resource utilization in terms of 
the percentage of physical resource block (PRB) used. Three interpretable groups emerge from the clustering process: %After 100 iterations, we divide our dataset into three interpretable groups: 
% The communication traffic can be affected by many factors such as the UE distribution, time of day, and system hardware. For this analysis, we consider the same factors used in state description of our MDP: (1) the number of active UEs, (2) network throughput, and (3) the bandwidth utilization in terms of the percentage of physical resource block (PRB) used. Using K-Means clustering on the daily traffic condition, we can divide our dataset into three interpretable groups:
% \textcolor{blue}{tianyu: I would just remove the "relatively" in all the items. In addition, I think figure 2 should be moved to this page.}
(Group 1) High traffic on the first cell; 
(Group 2) High traffic on the fourth cell;  and 
(Group 3) Low traffic in general.
Figure~\ref{fig:traffic_21_sec} shows how traffic varies across the 21 different traffic scenarios across these three groups. A cell has a high volume of traffic when it has a large number of active UEs, low throughput, and high utilization. 

%We conducted further analysis on the temporal aspect of the traffic condition for each group. %Figure~\ref{fig:avg_traffic_group} shows the traffic condition during low and high utilization hours. 
%We defined low utilization hours to be between midnight and 8 AM, which matches approximately to the time when most human consumers are inactive, and high utilization hours to be the other hours, when they are more likely to be actively accessing the network. From the figure, we observe that the magnitude of each traffic-related factor shifts significantly between the two time periods.

%\begin{figure}[ht]
%\centering
    % \subfigure[Average traffic.]{\includegraphics[width=\linewidth]{Figures/traffic_all_time_21sec.png}\label{fig:avg_traffic_group_all_time}}
%    \hspace{0.01\linewidth}
%    \subfigure[Average traffic during low utilization hours (0:00-8:00)]{\includegraphics[width=\linewidth]{Figures/traffic_non_peak_time_21sec.png}\label{fig:avg_traffic_group_non_peak}}
%    \hspace{0.01\linewidth}
 %   \subfigure[Average traffic during high utilization hours (8:00-24:00)]{\includegraphics[width=\linewidth]{Figures/traffic_peak_time_21sectors.png}\label{fig:avg_traffic_group_peak}}
 %   \caption{Average traffic over one week for each group at low and high utilization hours, illustrating the general daily traffic pattern shared across each group.}\label{fig:avg_traffic_group}
%\end{figure}

\begin{figure}[t]
\centering
\begin{tabular}{c}
\includegraphics[width=0.8\linewidth]{Figures/training-result-reward.png} \\
(a) Average reward on the training scenarios \\
~\\
\includegraphics[width=0.8\linewidth]{Figures/testing-result-reward.png} \\
(b) Average reward on the testing scenarios
\end{tabular}
\caption{Comparison of the average reward over 6 days. Our policy reuse framework with the policy selector (blue) achieves the closest performance to our upper bound BEST-$\pi$ (red) on average. For the training scenarios, it is exactly the same as BEST-$\pi$.}
\label{fig:reward_results}
\end{figure}

\subsection{Simulator}
\label{sec:simulator}
%\textcolor{gray}{Jimmy: Again, adding a high level sentence here would be good. Something like "Key to our experimental framework is a system-level simulator that allows our RL agent to collect interaction experiences for training...."} 
%A key to our experiments is the use of a communication network simulator to mimic real-world data, allowing our RL algorithm to interact with our collected traffic scenarios.
We use a proprietary system-level network simulator, as in~\cite{kang2021hrl}. 
%An example of a simulation scenario is shown in Figure~\ref{fig:sls}. 
This simulator emulates 4G/5G communication network behaviours, and supports various configurations that allow us to customize the traffic condition. In our experiment, we fix the number of base stations to 7, with one base station in the center of the layout. Each base station has 3 sectors and each sector has 4 cells with different carrier frequencies that are identical across all sectors and base stations. We vary the number and distribution of UEs, the packet size and request interval such that the simulation traffic condition at the north-east sector of the center base station matches  the real-world data presented. In our experiments, we aim to balance the load in this particular sector. Our RL policies are only aware of the control parameters and the traffic condition in this sector. 
%Our evaluation is also based on the performance of this sector.

To mimic real-world data, a fraction of the UEs are
% \textcolor{blue}{tianyu:it's what we do right? so just use "a portion of UEs IS ...", also remove the "the" before UEs.} 
uniformly concentrated at specified regions while the remaining are uniformly distributed across the environment. These dense traffic locations change at each hour. All UEs follow a random walk process with an average speed of 3~m/s. The packet arrival follows a Poisson process with variable size between 50~Kb to 2~Mb and inter-arrival time between 10 to 320~ms. Both are specified at each hour to create the desired traffic condition.
%\begin{figure}[ht]
%    \centering
%        \vspace{1mm}
%    \includegraphics[width=0.8\linewidth]{Figures/sls_simulator.png}
%    \caption{An example of a simulation scenario with 7 base stations, each with 3 sectors and 4 cells on each sector. Active and idle UEs connected to different cells are indicated by different shapes and colors.}
%    \label{fig:sls}
%\end{figure}

\subsection{Baselines}
\label{sec:baselines}
To showcase the effectiveness of the proposed method, we compare our solution with the following baselines: 
% \textcolor{gray}{tianyu: Maybe we should include the performance on learning from scratch to further showcase that we perform reasonably well, i.e. not too far away from the learning from scratch method.}
\textbf{Rule-based load balancing (BasicLB)} uses a fixed set of LB parameter values for all traffic scenarios. \textbf{Adaptive rule-based load balancing} (AdaptLB)~\cite{yang2012high} changes the LB parameter values based on the load status of the cells. \textbf{Random policy selection (RAND-$\pi$)} randomly selects a policy in the policy bank $\Pi$ at the beginning of every day. \textbf{Best policy selection (BEST-$\pi$)} selects the best policy based on the performance of all policies in $\Pi$ on the unseen scenarios in ${X}'$ for the whole week. \textbf{New policy trained on the unseen scenario (NEW-$\pi$)} directly trains a new RL policy on the unseen traffic scenario from scratch. BEST-$\pi$ is the best possible performance obtainable form one policy in the policy bank
%, as shown show in Figure~\ref{fig:rl_policy_21_sec_test} 
and it is not a feasible solution to deploy on a real network due to the use of exhaustive search. Similarly, NEW-$\pi$ is another upper bound on performance, and it is also not feasible if the RL agent is not allowed to learn from scratch on an unseen traffic scenario.


\subsection{Policy bank construction and analysis}
% \subsection{Policy bank analysis}
\label{sec:policy-bank-analysis}

%In this section, we conduct preliminary investigations on the performance of the RL policies in the policy bank
% \textcolor{blue}{tianyu: a "what" RL policy? maybe change it to "... performance of the constructed policy bank"?} 
%on unseen traffic scenarios. 
To ensure that our policy bank contains a diverse selection of policies trained from all types of traffic, we randomly select 3 traffic scenarios from each group introduced in Section~\ref{sec:traffic-analysis} to form our set of 9 training scenarios $\mathcal{X}$ and use the remaining 12 scenarios $\mathcal{X}'$ for testing. Following the formulation in Section~\ref{sec:rl-formulation}, we train one PPO policy for each $X\in \mathcal{X}$, creating a policy bank $\Pi$. The reward $R_t$ is the weighted average of the performance metrics defined in Section~\ref{sec:performance-metrics}.
% :
% \[
%     R_t = \frac{0.25}{10.7} G_{avg} + \frac{4}{4.9} G_{min} + \frac{0.5}{2.4(1+G_{sd})} + 0.2 G_{cong}.
% \]
% Because these metrics have values at different scales, we obtain these weights by searching exhaustively through a finite set of weight combinations and these weights were chosen due to their empirical performance for training an RL policy. 
% Note that we use the reciprocal of the shifted $G_{sd}$ so that maximizing the reward minimizes $G_{sd}$.
The weights are selected according to the empirical performance and they are correlated with the magnitude of the metrics. 
Note that we use the reciprocal of $G_{sd}$ so that maximizing the reward minimizes $G_{sd}$.
We also construct another RL policy $\tilde{\pi}$ trained on all scenarios in $\mathcal{X}$ for comparison. This is done by collecting interaction experience on each of the scenarios in parallel at each iteration in the learning process. All policies are trained for 200K interactions.
% with a decay $\lambda=0.97$. 
We use the PPO implementation in the Stable-Baseline 3~\cite{stable-baselines3} Python package. 

% The following was moved from the Method section:
We model the policy selector by a feed-forward neural network classifier with 3 hidden layers (with 128, 64, and 32 neurons, respectively), each preceded by a batch normalization and followed by a rectified linear unit activation. The output layer uses a softmax activation. The architecture hyperparameters were chosen using cross-validation.
% and 1 output layer.
% \textcolor{blue}{tianyu:is it 4 hidden layers or 3 layers with 1 output layer? I think maybe just be a bis specific here by saying "3 hidden layers and 1 output layer" to avoid confusion.)} 
% Each of the first three layers follows a batch normalization. The number of neurons for these layers are 128, 64 and 32, respectively.  
% \textcolor{gray}{tianyu: did we use cross validation to choose the network structure? if so maybe add it.} 
% We use rectified linear unit activation for the first three layers and softmax for the last layer. The number of layers, the number of neurons for each layer and the activation function were chosen using cross-validation.

%\textcolor{gray}{Jimmy: I feel the wording ``picking any policy" is not very clear, because it sounds like you are choosing a policy in the policy bank. I think it would be better to say something along the lines of ``the average performance of executing each policy in the policy bank on the target scenario"} 
Figure~\ref{fig:rl_policy_21_sec} illustrates the performance of executing each policy in the policy bank $\Pi$ in comparison with $\tilde{\pi}$ and the BasicLB method. We observe that, for some scenarios, the minimum possible average reward resulted from an RL policy in $\Pi$ lies
% \textcolor{blue}{tianyu: lies} 
much lower than the average reward resulted from the BasicLB. This supports the assumption that an RL policy trained on one scenario may not generalize well to another, and implies that randomly choosing a policy from the policy bank can significantly degrade the performance for some scenarios. On the other hand, the maximum possible average reward from an RL policy in $\Pi$ is always higher than the average reward resulted by $\tilde{\pi}$ and BasicLB even for the test scenarios. Furthermore, $\tilde{\pi}$ under-performs BasicLB for some test scenarios such as 12 and 14. This indicates that with careful selection of a policy trained from an individual scenario, we can achieve significant improvement over a policy trained on multiple scenarios and BasicLB. The next sections will present our results with the policy selector.



%\begin{figure}[ht]
%\centering
%    \hspace{0.01\linewidth}
%    \subfigure[Average reward on the training scenarios]{\includegraphics[width=\linewidth]{Figures/21sec-rl-analysis_train_group2.png}\label{fig:rl_policy_21_sec_train}}
%    \hspace{0.01\linewidth}
%    \subfigure[Average reward on the testing scenarios]{\includegraphics[width=\linewidth]{Figures/21sec-rl-analysis_test_group2.png}\label{fig:rl_policy_21_sec_test}}
    %\caption{Comparison of the average reward over one week for choosing any policy in the policy bank $\Pi$ against a policy $\tilde{\pi}$ trained on all scenarios in $\mathcal{X}$ and BasicLB. The blank line shows the minimum and maximum average reward.}
%    \caption{Comparison of the average reward over one week between policies in the policy bank $\Pi$ (orange), the policy $\tilde{\pi}$ trained on all scenarios in $\mathcal{X}$ (blue), and BasicLB (green) across training and testing scenarios. For the policy bank evaluation (orange), we show the mean, and indicate the minimum and maximum with error bars.}
%    \label{fig:rl_policy_21_sec}
%\end{figure}

%To further understand the correlation between the RL policy and the traffic condition, we conduct an  experiment that verifies whether policies trained on similar traffic conditions result in higher performance. The similarity between individual sectors' traffic patterns is non-trivial to define due to their high volatility. Hence, for simplicity, we use the L2 distance on the average traffic condition during the low and high utilization hours. Table~\ref{tab:similarity-performance} show the smallest number $k$ such that the policy trained on the $k$th most similar traffic scenario is within the top $k$ best performance for the unseen scenarios in $\mathcal{X}'$. Interestingly, we observe that group 2 has the smallest $k$ on average and group 1 has the largest $k$ on average. Referring back to Figure~\ref{fig:rl_policy_21_sec_test}, we see that any policy in $\Pi$ can easily outperform the rule-based method in a group 1 scenario, while it is much harder in a group 2 scenario. This demonstrates the benefit of selecting a policy based on the similarity of the traffic condition between the new scenario and the seen scenarios. 



%\begin{table}[!htbp]
%\centering
%\caption{The smallest number $k$ such that the policy trained on the $k$th most similar traffic scenario is within the top $k$ best performance for the unseen scenarios.}
%\label{tab:similarity-performance}
%\begin{tabular}{|c | c | c|  c | c | c |}
%\hline
%\multicolumn{2}{|c|}{\bf Group 1} & %\multicolumn{2}{c|}{\bf Group 2} &
%\multicolumn{2}{c|}{\bf Group 3}\\
%\hline
%Scenario  & $k$  & Scenario  & $k$  & Scenario &  $k$ %\\
%\hline
%3 & 3 & 8 & 1 & 16 & 1\\
%4 & 4 & 12 & 2 & 17 & 2 \\
%5 & 3 & 13 & 1 & 18 & 2 \\
%7 & 3 & 14 & 1 & 19 & 3\\
%\hline
%\end{tabular}
%\end{table}

==> ref.tex <==
 @techreport{ericsson_2022, url={https://www.ericsson.com/en/reports-and-papers/mobility-report/reports}, 
title={Ericsson Mobility Report},
 author={Ericsson},
 year={2022}} 
 
 @book{boyd2004convex,
  title={Convex optimization},
  author={Boyd, Stephen and Boyd, Stephen P and Vandenberghe, Lieven},
  year={2004},
  publisher={Cambridge university press}
}

 @article{jain1984quantitative,
  title={A quantitative measure of fairness and discrimination},
  author={Jain, Rajendra K and Chiu, Dah-Ming W and Hawe, William R and others},
  journal={Eastern Research Laboratory, Digital Equipment Corporation, Hudson, MA},
  volume={21},
  year={1984}
}
 
 @book{birge2011introduction,
  title={Introduction to stochastic programming},
  author={Birge, John R and Louveaux, Francois},
  year={2011},
  publisher={Springer Science \& Business Media}
}


@article{krokhmal2009random,
  title={Random assignment problems},
  author={Krokhmal, Pavlo A and Pardalos, Panos M},
  journal={European Journal of Operational Research},
  volume={194},
  number={1},
  pages={1--17},
  year={2009},
  publisher={Elsevier}
}
@article{cvxpy,
  author  = {Diamond, Steven and Boyd, Stephen},
  title   = {{CVXPY}: A Python-Embedded Modeling Language for Convex Optimization},
  journal = {Journal of Machine Learning Research},
  year    = {2016},
  volume  = {17},
  number  = {83},
  pages   = {1-5},
  url     = {http://jmlr.org/papers/v17/15-408.html}
}
@book{springer1979algebra,
  title={The Algebra of Random Variables},
  author={Springer, Mark D.},
  series={Wiley series in probability and mathematical statistics},
  publisher={John Wiley \& Sons},
  year={1979},
}

@techreport{3gpp.36.902,
 author = {3GPP},
 institution = {{3rd Generation Partnership Project (3GPP)}},
 note = {Version 9.2.0},
 number = {36.902},
 title = {{LTE; Evolved Universal Terrestrial Radio Access Network (E-UTRAN); Self-configuring and self-optimizing network (SON) use cases and solutions}},
 type = {Technical Specification (TS)},
 year = {2010}
}
@techreport{3gpp.36.331,
 author = {3GPP},
 institution = {{3rd Generation Partnership Project (3GPP)}},
 note = {Version 13.7.1},
 number = {36.331},
 title = {{LTE; 
Evolved Universal Terrestrial Radio Access (E-UTRA); 
Radio Resource Control (RRC); 
Protocol specification}},
 type = {Technical Specification (TS)},
 year = {2017}
}

@techreport{3gpp.38.300,
 author = {3GPP},
 institution = {{3rd Generation Partnership Project (3GPP)}},
 note = {Version 16.4.0},
 number = {38.300},
 title = {{5G;NR; NR and NG-RAN Overall description;Stage-2}},
 type = {Technical Specification (TS)},
 year = {2021}
}

@article{silver2018general,
  title={A general reinforcement learning algorithm that masters chess, shogi, and Go through self-play},
  author={Silver, David and Hubert, Thomas and Schrittwieser, Julian and Antonoglou, Ioannis and Lai, Matthew and Guez, Arthur and Lanctot, Marc and Sifre, Laurent and Kumaran, Dharshan and Graepel, Thore and others},
  journal={Science},
  volume={362},
  number={6419},
  pages={1140--1144},
  year={2018},
  publisher={American Association for the Advancement of Science}
}

@book{sutton2018reinforcement,
  title="{Reinforcement learning: An introduction}",
  author={Sutton, Richard S and Barto, Andrew G},
  year={2018},
  publisher={MIT press}
}
@article{xiong2019deep,
  title={Deep reinforcement learning for mobile 5g and beyond: Fundamentals, applications, and challenges},
  author={Xiong, Zehui et al},
  journal={IEEE Vehicular Technology Magazine},
  volume={14},
  number={2},
  pages={44--52},
  year={2019},
  publisher={IEEE}
}
@incollection{ng2006autonomous,
  title={Autonomous inverted helicopter flight via reinforcement learning},
  author={Ng, Andrew Y and Coates, et al},
  booktitle={Experimental robotics IX},
  pages={363--372},
  year={2006},
  publisher={Springer}
}
@article{lei2020deep,
  title={Deep reinforcement learning for autonomous internet of things: Model, applications and challenges},
  author={Lei, Lei et al},
  journal={IEEE Communications Surveys \& Tutorials},
  year={2020},
  publisher={IEEE}
}
@article{arulkumaran2017deep,
  title={Deep reinforcement learning: A brief survey},
  author={Arulkumaran, Kai and Deisenroth, et al},
  journal={IEEE Signal Processing Magazine},
  volume={34},
  number={6},
  pages={26--38},
  year={2017},
  publisher={IEEE}
}
@article{riedmiller2009reinforcement,
  title={Reinforcement learning for robot soccer},
  author={Riedmiller, Martin and Gabel, et al},
  journal={Autonomous Robots},
  volume={27},
  number={1},
  pages={55--73},
  year={2009},
  publisher={Springer}
}
@article{watkins1989learning,
  title={Learning from delayed rewards},
  author={Watkins, Christopher John Cornish Hellaby},
  year={1989},
  publisher={King's College, Cambridge United Kingdom}
}
@inproceedings{gordon1996stable,
  title={Stable fitted reinforcement learning},
  author={Gordon, Geoffrey J},
  booktitle={Advances in neural information processing systems},
  pages={1052--1058},
  year={1996}
}
@article{mnih2015human,
  title={Human-level control through deep reinforcement learning},
  author={Mnih, Volodymyr and Kavukcuoglu, et al},
  journal={nature},
  volume={518},
  number={7540},
  pages={529--533},
  year={2015},
  publisher={Nature Publishing Group}
}
@inproceedings{sutton2000policy,
  title={Policy gradient methods for reinforcement learning with function approximation},
  author={Sutton, Richard S and McAllester, et al},
  booktitle={Advances in neural information processing systems},
  pages={1057--1063},
  year={2000}
}


@phdthesis{sutton1984temporal,
  title={Temporal credit assignment in reinforcement learning},
  author={Sutton, Richard Stuart},
  year={1984},
  school={University of Massachusetts Amherst}
}
@article{hsu2020revisiting,
  title={Revisiting design choices in proximal policy optimization},
  author={Hsu, Chloe Ching-Yun and Mendler-D{\"u}nner, Celestine and Hardt, Moritz},
  journal={arXiv preprint arXiv:2009.10897},
  year={2020}
}
@inproceedings{schulman2015trust,
  title={Trust region policy optimization},
  author={Schulman, John and Levine, Sergey, et al},
  booktitle={International conference on machine learning},
  pages={1889--1897},
  year={2015},
  organization={PMLR}
}

@INPROCEEDINGS{mwanje2013qlearn,  author={Mwanje, Stephen S. and Mitschele-Thiel, Andreas},  booktitle={2013 IEEE 24th Annual International Symposium on Personal, Indoor, and Mobile Radio Communications (PIMRC)},   title={A Q-Learning strategy for LTE mobility Load Balancing},   year={2013},  volume={},  number={},  pages={2154-2158},  doi={10.1109/PIMRC.2013.6666500}}

@INPROCEEDINGS{kudo2014qlearn,  author={Kudo, Toshihito and Ohtsuki, Tomoaki},  booktitle={2014 IEEE 80th Vehicular Technology Conference (VTC2014-Fall)},   title={Q-Learning Based Cell Selection for UE Outage Reduction in Heterogeneous Networks},   year={2014},  volume={},  number={},  pages={1-5},  doi={10.1109/VTCFall.2014.6966140}}

@article{nasri2013handover,
  title={Handover adaptation for dynamic load balancing in 3GPP long term evolution systems},
  author={Nasri, Ridha and Altman, Zwi},
  journal={International Conference on Advances in Mobile Computing and Multimedia},
  year={2007}
}
@article{alsuhli2021mobility,
  title={Mobility load management in cellular networks: A deep reinforcement learning approach},
  author={Alsuhli, Ghada and Banawan, Karim and Attiah, Kareem and Elezabi, Ayman and Seddik, Karim and Gaber, Ayman and Zaki, Mohamed and Gadallah, Yasser},
  journal={IEEE Transactions on Mobile Computing},
  year={2021},
  publisher={IEEE}
}
@inproceedings{huang2015threshold,
  title={A threshold-based multi-traffic load balance mechanism in LTE-A networks},
  author={Huang, Zhangpeng and Liu, Jing and Shen, Qiang and Wu, Jin and Gan, Xiaoying},
  booktitle={2015 IEEE wireless communications and networking conference (WCNC)},
  pages={1273--1278},
  year={2015},
  organization={IEEE}
}
@inproceedings{addali2020mobility,
  title={Mobility load balancing with handover minimization for 5G small cell networks},
  author={Addali, Khaled M and Chang, Zhengwei and Lu, Jizhao and Liu, Rongke and Kadoch, Michel},
  booktitle={2020 International Wireless Communications and Mobile Computing (IWCMC)},
  pages={1222--1227},
  year={2020},
  organization={IEEE}
}

@INPROCEEDINGS{li2005umts,
  author={Jing Li and Chen Fan and Dacheng Yang and Jian Gu},
  booktitle={VTC-2005-Fall. 2005 IEEE 62nd Vehicular Technology Conference, 2005.}, 
  title={Umts soft handover algorithm with adaptive thresholds for load balancing}, 
  year={2005},
  volume={4},
  number={},
  pages={2508-2512},
  doi={10.1109/VETECF.2005.1559001}}

@INPROCEEDINGS{viering2009math,
  author={Viering, I. and Dottling, M. and Lobinger, A.},
  booktitle={2009 IEEE International Conference on Communications}, 
  title={A Mathematical Perspective of Self-Optimizing Wireless Networks}, 
  year={2009},
  volume={},
  number={},
  pages={1-6},
  doi={10.1109/ICC.2009.5198628}}

@INPROCEEDINGS{jansen2010handover,  author={Jansen, Thomas and Balan, Irina, et al},  booktitle={2010 IEEE 72nd Vehicular Technology Conference - Fall},   title={Handover Parameter Optimization in LTE Self-Organizing Networks},   year={2010},  volume={},  number={},  pages={1-5},  doi={10.1109/VETECF.2010.5594245}}

@INPROCEEDINGS{kwan2010on,  author={Kwan, Raymond and Arnott, Rob and Paterson, Robert and Trivisonno, Riccardo and Kubota, Mitsuhiro},  booktitle={2010 IEEE 72nd Vehicular Technology Conference - Fall},   title={On Mobility Load Balancing for LTE Systems},   year={2010},  volume={},  number={},  pages={1-5},  doi={10.1109/VETECF.2010.5594565}}

@INPROCEEDINGS{ali2007directional,
  author={Ali, Khaled A. and Hassanein, Hossam S. and Mouftah, Hussein T.},
  booktitle={2007 12th IEEE Symposium on Computers and Communications}, 
  title={Directional Cell Breathing Based Reactive Congestion Control in WCDMA Cellular Networks}, 
  year={2007},
  volume={},
  number={},
  pages={685-690},
  doi={10.1109/ISCC.2007.4381553}}
  
@misc{nec2009son,
author={NEC}, title={Self Organizing Network: NEC’s Proposals for Next-Generation Radio Network Management}, month={February},
year={2009}, note={http://www.nec.com}
}

@ARTICLE{hu2010self,  author={Hu, Honglin and Zhang, Jian, et al},  journal={IEEE Communications Magazine},   title={Self-configuration and self-optimization for LTE networks},   year={2010},  volume={48},  number={2},  pages={94-100},  doi={10.1109/MCOM.2010.5402670}}

@INPROCEEDINGS{yang2012high,  author={Yang, Ying and Li, Pengfei, et alg},  booktitle={2012 IEEE Vehicular Technology Conference (VTC Fall)},   title={A High-Efficient Algorithm of Mobile Load Balancing in LTE System},   year={2012},  volume={},  number={},  pages={1-5},  doi={10.1109/VTCFall.2012.6398873}}

@INPROCEEDINGS{munoz2011optimization,  author={Muñoz, P. and Barco, R., et al},  booktitle={2011 IEEE 73rd Vehicular Technology Conference (VTC Spring)},   title={Optimization of a Fuzzy Logic Controller for Handover-Based Load Balancing},   year={2011},  volume={},  number={},  pages={1-5},  doi={10.1109/VETECS.2011.5956148}}

@INPROCEEDINGS{tolli2002performance,  author={Tolli, A. and Hakalin, P. and Holma, H.},  booktitle={2002 IEEE International Conference on Communications. Conference Proceedings. ICC 2002 (Cat. No.02CH37333)},   title={Performance evaluation of common radio resource management (CRRM)},   year={2002},  volume={5},  number={},  pages={3429-3433 vol.5},  doi={10.1109/ICC.2002.997467}}

@INPROCEEDINGS{tolli2002adaptive,  author={Tolli, A. and Hakalin, P.},  booktitle={Proceedings IEEE 56th Vehicular Technology Conference},   title={Adaptive load balancing between multiple cell layers},   year={2002},  volume={3},  number={},  pages={1691-1695 vol.3},  doi={10.1109/VETECF.2002.1040504}}

@article{wiering2008ensemble,
  title={Ensemble algorithms in reinforcement learning},
  author={Wiering, Marco A and Van Hasselt, Hado},
  journal={IEEE Transactions on Systems, Man, and Cybernetics, Part B (Cybernetics)},
  volume={38},
  number={4},
  pages={930--936},
  year={2008},
  publisher={IEEE}
}

@article{saphal2020seerl,
  title={Seerl: Sample efficient ensemble reinforcement learning},
  author={Saphal, Rohan and Ravindran, Balaraman, et al},
  journal={arXiv preprint arXiv:2001.05209},
  year={2020}
}

@BOOK{hto,
  TITLE = {LTE Advanced: 3GPP Solution for IMT-Advanced},
  SUBTITLE = {},
  AUTHOR = {Holma H and Toskala A},
  YEAR = {2012},
  PUBLISHER = {John Wiley and Sons},
}

@article{samdanis2020road,
  title={The road beyond 5G: A vision and insight of the key technologies},
  author={Samdanis, Konstantinos and Taleb, Tarik},
  journal={IEEE Network},
  volume={34},
  number={2},
  pages={135--141},
  year={2020},
  publisher={IEEE}
}

@article{zheng2020reliable,
  title={A Reliable Communication and Load Balancing Scheme for Resource-Limited Networks},
  author={Zheng, Xiuping and Idrees, Asma, et al},
  journal={IEEE Access},
  volume={8},
  pages={179921--179930},
  year={2020},
  publisher={IEEE}
}


@article{schulman2017proximal,
  title={Proximal policy optimization algorithms},
  author={Schulman, John and Wolski, Filip and Dhariwal, Prafulla and Radford, Alec and Klimov, Oleg},
  journal={arXiv preprint arXiv:1707.06347},
  year={2017}
}

@inproceedings{kang2021hrl, 
    title={Hierarchical Policy Learning for Hybrid Communication Load Balancing},
    author={Kang, Jikun and Chen, Xi and Wu, Di and Xu, Yi Tian and Liu, Xue and Dudek, Gregory and Lee, Taeseop and Park, Intaik} , 
    booktitle={2021 IEEE international conference on communications},
    year={2021},
    organization={IEEE}
 }
@inproceedings{wu2021load,
  title={Load Balancing for Communication Networks via Data-Efficient Deep Reinforcement Learning},
  author={Wu, Di and Kang, Jikun and Xu, Yi Tian and Li, Hang and Li, Jimmy and Chen, Xi and Rivkin, Dmitriy and Jenkin, Michael and Lee, Taeseop and Park, Intaik and others},
  booktitle={2021 IEEE Global Communications Conference (GLOBECOM)},
  pages={01--07},
  year={2021},
  organization={IEEE}
}
@inproceedings{li2022traffic,
  title={Traffic Scenario Clustering and Load Balancing with Distilled Reinforcement Learning Policies},
  author={Li, Jimmy and Wu, Di and Xu, Yi Tian and Li, Tianyu and Jang, Seowoo and Liu, Xue and Dudek, Gregory},
  booktitle={ICC 2022-IEEE International Conference on Communications},
  pages={1536--1541},
  year={2022},
  organization={IEEE}
}
 
 @article{xu2019load,
  title={Load balancing for ultradense networks: A deep reinforcement learning-based approach},
  author={Xu, Yue and Xu, Wenjun, et al},
  journal={IEEE Internet of Things Journal},
  volume={6},
  number={6},
  pages={9399--9412},
  year={2019},
  publisher={IEEE}
}


@article{munoz2012fuzzy,
  title={Fuzzy rule-based reinforcement learning for load balancing techniques in enterprise LTE femtocells},
  author={Mu{\~n}oz, Pablo and Barco, Raquel and Ruiz-Avil{\'e}s, Jos{\'e} Mar{\'\i}a and De La Bandera, Isabel and Aguilar, Alejandro},
  journal={IEEE Transactions on Vehicular Technology},
  volume={62},
  number={5},
  pages={1962--1973},
  year={2013},
  publisher={IEEE}
}

@article{mwanje2016cognitive,
  title={Cognitive cellular networks: A Q-learning framework for self-organizing networks},
  author={Mwanje, Stephen S and Schmelz, Lars Christoph and Mitschele-Thiel, Andreas},
  journal={IEEE Transactions on Network and Service Management},
  volume={13},
  number={1},
  pages={85--98},
  year={2016},
  publisher={IEEE}
}


@inproceedings{lu2017expressive,
  title={The expressive power of neural networks: A view from the width},
  author={Lu, Zhou and Pu, Hongming and Wang, Feicheng and Hu, Zhiqiang and Wang, Liwei},
  booktitle={Proceedings of the 31st International Conference on Neural Information Processing Systems},
  pages={6232--6240},
  year={2017}
}

@inproceedings{DBLP:conf/vtc/KwanAPTK10,
  author    = {Raymond Kwan and
               Rob Arnott and
               Robert Paterson and
               Riccardo Trivisonno and
               Mitsuhiro Kubota},
  title     = {On Mobility Load Balancing for {LTE} Systems},
  booktitle = {{VTC} Fall},
  pages     = {1--5},
  publisher = {{IEEE}},
  year      = {2010}
}

@misc{stable-baselines3,
  author = {Raffin, Antonin and Hill, Ashley and Ernestus, Maximilian and Gleave, Adam and Kanervisto, Anssi and Dormann, Noah},
  title = {Stable Baselines3},
  year = {2019},
  publisher = {GitHub},
  journal = {GitHub repository},
  howpublished = {\url{https://github.com/DLR-RM/stable-baselines3}},
}

  
@article{feriani2022multiobjective,
  title={Multiobjective load balancing for multiband downlink cellular networks: A meta-reinforcement learning approach},
  author={Feriani, Amal et al},
  journal={IEEE Journal on Selected Areas in Communications},
  volume={40},
  number={9},
  pages={2614--2629},
  year={2022},
  publisher={IEEE}
}
@inproceedings{ma2022coordinated,
  title={Coordinated Load Balancing in Mobile Edge Computing Network: a Multi-Agent DRL Approach},
  author={Ma, Manyou and Wu, Di and Xu, Yi Tian and Li, Jimmy and Jang, Seowoo and Liu, Xue and Dudek, Gregory},
  booktitle={ICC 2022-IEEE International Conference on Communications},
  pages={619--624},
  year={2022},
  organization={IEEE}
}

@inproceedings{kang2021hierarchical,
  title={Hierarchical policy learning for hybrid communication load balancing},
  author={Kang, Jikun and Chen, Xi and Wu, Di and Xu, Yi Tian and Liu, Xue and Dudek, Gregory and Lee, Taeseop and Park, Intaik},
  booktitle={ICC 2021-IEEE International Conference on Communications},
  pages={1--6},
  year={2021},
  organization={IEEE}
}

@inproceedings{li2022traffic,
  title={Traffic scenario clustering and load balancing with distilled reinforcement learning policies},
  author={Li, Jimmy and Wu, Di and Xu, Yi Tian and Li, Tianyu and Jang, Seowoo and Liu, Xue and Dudek, Gregory},
  booktitle={ICC 2022-IEEE International Conference on Communications},
  pages={1536--1541},
  year={2022},
  organization={IEEE}
}

@article{zhang2022metaems,
  title={MetaEMS: A Meta Reinforcement Learning-based Control Framework for Building Energy Management System},
  author={Zhang, Huiliang and Wu, Di and Boulet, Benoit},
  journal={arXiv preprint arXiv:2210.12590},
  year={2022}
}

@article{wu2018optimizing,
  title={Optimizing home energy management and electric vehicle charging with reinforcement learning},
journal={ICML 2018 Workshop on machine learning for climate change},
  author={Wu, Di and Rabusseau, Guillaume and Fran{\c{c}}ois-lavet, Vincent and Precup, Doina and Boulet, Benoit}

    year={2018}
}

@book{wu2018machine,
  title={Machine learning algorithms and applications for sustainable smart grid},
  author={Wu, Di},
  year={2018},
  publisher={McGill University (Canada)}
}

@article{huang2021modellight,
  title={Modellight: Model-based meta-reinforcement learning for traffic signal control},
  author={Huang, Xingshuai and Wu, Di and Jenkin, Michael and Boulet, Benoit},
  journal={arXiv preprint arXiv:2111.08067},
  year={2021}
}

@inproceedings{fucloser,
  title={A Closer Look at Offline RL Agents},
  author={Fu, Yuwei and Wu, Di and Boulet, Benoit},
  booktitle={Advances in Neural Information Processing Systems}
}

@inproceedings{fu2022reinforcement,
  title={Reinforcement learning based dynamic model combination for time series forecasting},
  author={Fu, Yuwei and Wu, Di and Boulet, Benoit},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={36},
  number={6},
  pages={6639--6647},
  year={2022}
}

@article{wu2019multiple,
  title={Multiple kernel learning-based transfer regression for electric load forecasting},
  author={Wu, Di and Wang, Boyu and Precup, Doina and Boulet, Benoit},
  journal={IEEE Transactions on Smart Grid},
  volume={11},
  number={2},
  pages={1183--1192},
  year={2019},
  publisher={IEEE}
}
@inproceedings{wu2017boosting,
  title={Boosting based multiple kernel learning and transfer regression for electricity load forecasting},
  author={Wu, Di and Wang, Boyu and Precup, Doina and Boulet, Benoit},
  booktitle={Machine Learning and Knowledge Discovery in Databases: European Conference, ECML PKDD 2017, Skopje, Macedonia, September 18--22, 2017, Proceedings, Part III 10},
  pages={39--51},
  year={2017},
  organization={Springer}
}
@article{feriani2022multiobjective,
  title={Multiobjective load balancing for multiband downlink cellular networks: A meta-reinforcement learning approach},
  author={Feriani, Amal and Wu, Di and Xu, Yi Tian and Li, Jimmy and Jang, Seowoo and Hossain, Ekram and Liu, Xue and Dudek, Gregory},
  journal={IEEE Journal on Selected Areas in Communications},
  volume={40},
  number={9},
  pages={2614--2629},
  year={2022},
  publisher={IEEE}
}

@inproceedings{kang2021hierarchical,
  title={Hierarchical policy learning for hybrid communication load balancing},
  author={Kang, Jikun and Chen, Xi and Wu, Di and Xu, Yi Tian and Liu, Xue and Dudek, Gregory and Lee, Taeseop and Park, Intaik},
  booktitle={ICC 2021-IEEE International Conference on Communications},
  pages={1--6},
  year={2021},
  organization={IEEE}
}

@inproceedings{DBLP:conf/ijcai/LinW21,
  author    = {Weixuan Lin and
               Di Wu},
  title     = {Residential Electric Load Forecasting via Attentive Transfer of Graph
               Neural Networks},
  booktitle = {{IJCAI}},
  pages     = {2716--2722},
  publisher = {ijcai.org},
  year      = {2021}
}

@inproceedings{wu2022short,
  title={Short-term load forecasting with deep boosting transfer regression},
  author={Wu, Di and Xu, Yi Tian and Jenkin, Michael and Wang, Ju and Li, Hang and Liu, Xue and Dudek, Gregory},
  booktitle={ICC 2022-IEEE International Conference on Communications},
  pages={5530--5536},
  year={2022},
  organization={IEEE}
}

@article{wu2022efficient,
  title={Efficient residential electric load forecasting via transfer learning and graph neural networks},
  author={Wu, Di and Lin, Weixuan},
  journal={IEEE Transactions on Smart Grid},
  year={2022},
  publisher={IEEE}
}

==> related-works.tex <==
\section{Related Work}\label{related-works}
% In this section, we discuss the relevant prior arts in load balancing. 
%- Early work: benefits of load balancing identified in \cite{tolli2002performance, tolli2002adaptive}
Load balancing has long been identified as a crucial aspect of radio resource management \cite{tolli2002performance, tolli2002adaptive}. Typically, load balancing aims to improve throughput, ensure fairness, reduce latency, while also minimizing the number of handovers \cite{hu2010self}. Load balancing has often been studied under the larger umbrella of self-organizing networks (SON), which aims to provide a holistic framework for self-configuration, self-optimization, and self-healing, with load balancing being a key topic within self-optimization \cite{hu2010self}.  The inclusion of SON as part of the standard 3GPP Long Term Evolution (LTE) specifications has further accelerated the research effort in load balancing in recent years \cite{nec2009son}.

%- self-organizing network (SON) and LTE \cite{nec2009son} \cite{hu2010self}. Self optimization is a key aspect of SON. 
%MLB is an important topic in self-optimization, which uses handovers to balance the network load among cells and base stations. 

Rule-based load balancing has been the dominant approach over the last few decades. Popular approaches include the adjustment of the coverage area of various cells \cite{ali2007directional, li2005umts,viering2009math}, as well as the adjustment of handover parameters that affect the cell selection criteria of user equipment (UEs) \cite{jansen2010handover,kwan2010on,yang2012high,nasri2013handover}. Along this latter direction, Kwan \emph{et al.} has introduced a method for adjusting cell-specific offsets between neighboring cells at constant step sizes based on the cell load \cite{kwan2010on}. Yang \emph{et al.} further proposes a technique for computing the step size adaptively, so as to balance cell loads more efficiently. Other load balancing approaches that have been studied include the minimization of the number of handovers \cite{hu2010self}, and the tuning of hysteresis and time-to-trigger parameters \cite{jansen2010handover}

%Handover parameter tuning \cite{jansen2010handover}
%-  Adjustment of coverage area \cite{ali2007directional}, \cite{li2005umts}, \cite{viering2009math}
%- A body of work on adjustment of the handover region \cite{nasri2013handover}. 
%Adjust cell-specific offset between neighboring cells. Adjust offset at constant step-sizes based on cell load\cite{kwan2010on}. To improve efficiency, propose adaptive step size to more efficiently balance the load \cite{yang2012high}.

%- Other approaches minimize number of handovers \cite{hu2010self}, and tune the hysteresis and time-to-trigger parameters \cite{jansen2010handover}

The application of reinforcement learning (RL) is an active area of research, especially with the recent development of deep RL \cite{mnih2015human, silver2018general}. Q-learning \cite{watkins1989learning} is a popular choice among the various reinforcement learning methods, since it does not require the explicit modelling system dynamics, and the expected utility of each control action can be easily extracted. Munoz \emph{et al.} use Q-learning to find the optimal parameters for a fuzzy logic controller that adjusts load balancing parameters \cite{munoz2011optimization}.
Mwanje \emph{et al.} use Q-learning to adaptively tune the step size of cell-specific offsets based on the load condition \cite{mwanje2013qlearn}.  While these lines of work achieve load balancing by controlling the serving cells, the optimization of UE behavior has also been studied. Kudo \emph{et al.} apply Q-learning from the perspective of UEs to determine to which cells to send service requests in order to minimize outage \cite{kudo2014qlearn}. In contrast to these prior work, this paper focuses on addressing challenges related to variations in traffic patterns across different cells. Our method selects the most suitable RL policy from a policy bank based on network measurements, which allows our system to achieve significant improvement over rule-based methods in unseen traffic scenarios.
